SocraSynth: Multi-LLM Reasoning with Conditional Statistics

Large language models (LLMs), while promising, face criticisms for biases, hallucinations, and a lack of reasoning capability. This paper introduces SocraSynth, a multi-LLM agent reasoning platform developed to mitigate these issues. SocraSynth utilizes conditional statistics and systematic context enhancement through continuous arguments, alongside adjustable debate contentiousness levels. The platform typically involves a human moderator and two LLM agents representing opposing viewpoints on a given subject. SocraSynth operates in two main phases: knowledge generation and reasoning evaluation. In the knowledge generation phase, the moderator defines the debate topic and contentiousness level, prompting the agents to formulate supporting arguments for their respective stances. The reasoning evaluation phase then employs Socratic reasoning and formal logic principles to appraise the quality of the arguments presented. The dialogue concludes with the moderator adjusting the contentiousness from confrontational to collaborative, gathering final, conciliatory remarks to aid in human reasoning and decision-making. Through case studies in three distinct application domains, this paper showcases SocraSynth's effectiveness in fostering rigorous research, dynamic reasoning, comprehensive assessment, and enhanced collaboration. This underscores the value of multi-agent interactions in leveraging LLMs for advanced knowledge extraction and decision-making support.

==> CRIT-Algorithm.tex <==

\section{Evaluation with CRIT}
\label{sec-CRIT}

This section summarizes the CRIT (Critical Reading Template) method
that we proposed 
\cite{SocreticMethodChang2023,CRIT-Extended} for evaluating 
the validity of a document's claim. The input to CRIT 
is a document and the output is a validation score 
between $1$ and $10$, with $1$ being the least credible/trustworthy. 

Formally, given document $d$, CRIT performs
evaluation and produces score $\Gamma$.
Let $\Omega$ denote the claim of $d$, and $R$ a set of reasons supporting the claim.  
Furthermore, we define ($\gamma_r, \theta_r$) = V($r \Rightarrow \Omega$) as
the causal validation function, where 
$\gamma_r$ denotes the validation score for reason $r \in R$, and
$\theta_r$ source credibility. 
Table~\ref{tab:CRIT} presents the pseudo-code of 
$\Gamma$ = CRIT($d$), generating the final validation score $\Gamma$ for
document $d$ with justifications.

We can treat the stance of the proponent
and opponent of a debate as their respective conclusion.
Using our example in Section~\ref{sec-debate}, the conclusion 
of Agent A is ``Supporting regulating the use of large language
models in education and research,'' and the conclusion of Agent B is 
``Opposing regulating the use of large language
models in education and research.''
Together with each agent's arguments in several rounds of debate
are readily for CRIT to conduct evaluation.  

\subsection{What? Locating Conclusion}

As shown in the pseudocode in Table~\ref{tab:CRIT}, 
the CRIT algorithm starts in
its step $\#1$, asking GPT-4 to identify the conclusion of a document. To avoid any misunderstandings, the prompt includes a clear instruction and definition. (In the square brackets, {\em in} denotes a input slot to an LLM and {\em out} the output slot.)

\begin{table}[ht!]
\small
\begin{tabular}{p{0.6cm}|p{7.0cm}}
p1.1 & ``What is the conclusion in document [in: $d$] 
  [out: $\Omega$]? \\ 
& The conclusion statement may 
  be written in the last paragraph, near 
  keywords `in conclusion,' `in summary,' or `therefore.''' \\
\end{tabular}
\vspace{-.05in}
\end{table}

\begin{table}[ht!]
\vspace{-.05in}
\begin{small}
\begin{center}
\begin{tikzpicture}
\node (table) [inner sep=0pt] {
\begin{tabular}{|p{0.56cm}|p{6.9cm}|}
\toprule
\textbf{} & \textbf{Function $\Gamma$ = CRIT($d$)} \\
\midrule
%& Function $\Gamma$ = CRIT($d$); \\
& \textbf{Input}. $d$: document; \textbf{Output}. $\Gamma$: validation score; \\
& \textbf{Vars}. $\Omega$: claim; $R$ \& $R'$: reason \& counter reason set; \\
& \textbf{Subroutines}. $Claim$(), $FindDoc$(), $Validate$(); \\
& \textbf{Begin} \\
\#1 & {\hspace{.2cm}}Identify in $d$ the claim statement $\Omega$; \\
\#2 & {\hspace{.2cm}}Find a set of supporting reasons $R$ to $\Omega$; \\
\#3 & {\hspace{.2cm}}For $r \in R$ eval $r \Rightarrow \Omega$ \\
& {\hspace{.5cm}}{If} $Claim$($r$), ($\gamma_r$, $\theta_r$) = CRIT($FindDoc$($r$)); \\
& {\hspace{.5cm}}{else}, ($\gamma_r$, $\theta_r$) = $V$($r \Rightarrow \Omega$); \\
%\#4 & {\hspace{.2cm}}Assessing rival arguments: \\
\#4 & {\hspace{.2cm}}Find a set of rival reasons $R'$ to $\Omega$; \\
\#5 & {\hspace{.2cm}}For $r' \in R'$, ($\gamma_{r'}$, $\theta_{r'}$) = V($r' \Rightarrow \Omega$) eval rivals; \\
\#6 & {\hspace{.2cm}}Compute weighted sum $\Gamma$, with $\gamma_r$, $\theta_r$, $\gamma_{r'}$, $\theta_{r'}$. \\
\#7 & {\hspace{.2cm}}Analyze the arguments to arrive at the $\Gamma$ score. \\
\#8 & {\hspace{.2cm}}Reflect on and synthesize CRIT in other contexts. \\
& \textbf{End} \\
\bottomrule
\end{tabular}
};
\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
\end{tikzpicture}
\vspace{.05in}
\caption{CRIT Pseudo-code. (The symbol ``$\Rightarrow$'' can be  used for either inductive and deductive reasoning.)}
\label{tab:CRIT}
\end{center}
\end{small}
\vspace{-.2in}
\end{table}

\subsection{Why? Finding Reasons of Conclusion}

Reasons are explanations for why we should believe in a claim. To justify a claim, such as ``The Earth is the center of the universe,'' supporting evidence must be provided. Whether someone can be convinced of the claim depends on the validity of the evidence, both theoretical and empirical. If the evidence is logical and comprehensive, it may lead to belief in the claim. However, if some of the supporting reasons can be refuted, then the claim is on uncertain footing. 

Step $\#2$ in Table~\ref{tab:CRIT} prompts GPT-4 to find a set of supporting reasons $R$. To further enhance the accuracy and comprehensiveness of the results, the prompt can ask for not only ``reasons'' but also ``evidences'' or ``opinions'' to query for the document's support to its conclusion, similar to the ensemble method.

\begin{table}[ht!]
\small
\begin{tabular}{p{0.6cm}|p{7.0cm}}
p2 & ``What are the supporting reasons [out: $R$] of conclusion \\
& [in: $\Omega$] of [in: $d$]? A reason can be evidence or opinion.'' 
\end{tabular}
\vspace{-.1in}
\end{table}

\subsection{Evaluate Reason-Conclusion Pair}
\label{sec:validation}

The task of Validate($r \Rightarrow \Omega$) is to evaluate the validity of the reason $r$ as justification for the conclusion $\Omega$. It is important to note that this reasoning justification can be inductive, deductive, or abductive. While the symbol $\Rightarrow$ can be used for all three types of reasoning, the underlying reasoning mechanisms are different. Bayesian methods are more appropriate for inductive reasoning, where probability estimates and updating beliefs based on new evidence play a central role. Deductive reasoning relies on a set of logical rules to arrive at a certain conclusion based on given premises, without any need for statistical inference or probability estimates. Abductive reason is speculative in
nature, and should not be used to justify an argument.

CRIT issues four prompts in step $\#3$ to evaluate the reasoning validity and source credibility of each $r \in R$ for the $r \Rightarrow \Omega$ argument. It first elicits supporting evidence for reason $r \in R$. This evidence can be a theory, an opinion, statistics, or a claim obtained from other sources. If the reason itself is a claim, then the sources that the claim is based on are recursively examined. The strength of the argument and its source credibility are rated on a scale of $1$ to $10$, with $10$ being the strongest.

\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.0cm}}
%p3 & For each $r \in R$ \\
p3.1 & ``What is the evidence for reason [in: $r$] to support
conclusion [in: $\Omega$] in document [in: $d$]? [out: evidence]'' \\ 
p3.2 & ``What is the type of evidence? A) theory, B) opinion, C) statistics, or {\color{red}D}) claim from other sources? [in: evidence] [out: type]'' \\
p3.3 & ``If the type [in: type] is {\color{red}D}), call CRIT recursively'' \\
p3.4 & ``How strongly does reason [in: $r$] support
  [in: $\Omega$] in document [in: $d$]? Rate argument validity [out: $\gamma_r$] and source credibility [out: $\theta_r$] between $1$ and $10$ (strongest).''
\end{tabular}
\vspace{-.2in}
\end{table}

\subsection{Prompt Counter Arguments}
\label{sec:counter}

For a monologue, 
CRIT relies on GPT-4 to generate and
evaluate counter arguments, similar to
how it prompts GPT-4 to extract and 
evaluate reasons. 
CRIT in its step $\#4$ asks GPT-4 to provide missing
rival reasons, and then pair rival reasons
with the conclusion to conduct validation.

In a dialogue setting counter-arguments are arguments
of the opponent. Therefore, in our SocraSynth debate 
scenario, the counter-arguments can be extracted from
the opponent's arguments.

\begin{table}[th!]
\small
\begin{tabular}{p{0.6cm}|p{7.0cm}}
p4 & ``Are there counterarguments against [in: $r \Rightarrow \Omega$]? If so, provide counter reasons [output $R'$].'' \\
p5 & Similar to p3, except for replacing reason $r$ with rival $r'$.
\end{tabular}
\vspace{-.2in}
\end{table}

\subsection{Recursive Consideration}

The pseudocode presented in Table~\ref{tab:CRIT}
shows that step $3$ can call CRIT recursively. This is because if a reason is itself a conclusion or a quote drawn from
some other documents, CRIT can find reasons from those documents and then perform an aggregated validation.

Next, in step $\#6$, CRIT computes an aggregated score by performing a weighted sum on the validation multiplied by the credibility scores of both arguments and counterarguments, and then outputs the final assessment score $\Gamma$.

\begin{table}[ht!]
\small
\begin{tabular}{p{0.6cm}|p{7.0cm}}
p6 & ``Final score [out: $\Gamma$]. $\Gamma = 
\sum_{r \in R \cup R'} \gamma_r \times \theta_r / |R \cup R'|$.
\end{tabular}
\vspace{-.1in}
\end{table}

The final validation score is calculated as the sum of the validity score, weighted by the credibility of the sources, when available. 

==> FunctionValidate.tex <==
\subsection{Recursive Consideration}

The pseudocode presented in Table~\ref{tab:CRIT}
shows that step $3$ can call CRIT recursively. This is because if a reason is itself a conclusion or a quote drawn from
some other documents, CRIT can find reasons from those documents and then perform an aggregated validation.

Next, in step $\#6$, CRIT computes an aggregated score by performing a weighted sum on the validation multiplied by the credibility scores of both arguments and counterarguments, and then outputs the final assessment score $\Gamma$.

\begin{table}[ht!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p6 & ``Final score [out: $\Gamma$]. $\Gamma = 
\sum_{r \in R \cup R'} \gamma_r \times \theta_r / |R \cup R'|$.
\end{tabular}
\vspace{-.1in}
\end{table}

The final validation score is calculated as the sum of the validity score, weighted by the credibility of the sources. This yields a score of $75\%$. Source credibility can be modeled in a manner similar to PageRank~\cite{PageRank1998}.

\subsection{Student Practice}

Continuing with GRIT, once the text has been scored in step $\#6$, it can be valuable for readers or students to enhance their analytical and writing skills by summarizing and analyzing the justifications produced by GPT-3. CRIT in its step $\#7$ can prompt GPT-3 to generate a report, which readers and students can then compare with their own answered guided by GRIT.

\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p7 & ``For every $r \in R \cup R'$ justify the validity score $\gamma_r$ and source credibility score $\theta_r$ for $r \Rightarrow \Omega$ reasoning.''
\end{tabular}
\vspace{-.2in}
\end{table}

\subsection{Counterfactual Reasoning}
\label{sec:cf}


The final step of GRIT involves using the counterfactual method \cite{WinArgument2006,Cross-Examination2021} to encourage students to reconsider the arguments and counterarguments presented in the text based on new contextual information. CRIT can prompt students with questions such as ``what if the debate in the text took place now instead of in the 1950s?'' or ``what if the main event in the text occurred in Asia instead of in Europe?'' Students can express their own opinions and findings based on further reading with different contextual settings
such as people, location and time, and challenge the conclusions drawn in the text. 

\begin{table}[h!]
\small
\begin{tabular}{p{0.6cm}|p{7.2cm}}
p8 & ``For every $r \in R \cup R'$, evaluate $r \Rightarrow \Omega$
in [in context].''
\end{tabular}
\vspace{-.25in}
\end{table}









==> IntroICML.tex <==
\section{Introduction}
\label{sec-intro}




\begin{enumerate}
\item Focused Presentation: Each LLM presents its core argument concisely, leveraging its extensive knowledge base.
\item Critical Analysis: The mediator prompts LLMs to critically analyze each other's arguments, focusing on {\em evidence} and {\em logic} rather than volume of information.
\item Synthesis Round: LLMs synthesize insights from the debate, acknowledging valid points from the opposing view.
\item Concluding Insights: The mediator summarizes key takeaways, emphasizing new insights and potential areas for further exploration.
\end{enumerate}












Deciding on the multifaceted perspectives of a subject matter impartially is a complex task. Philosophically, one could rely on methods like dialectical reasoning, which involves examining and synthesizing opposing views. Algorithmically, one approach could involve analyzing a wide array of data sources to identify common and divergent themes related to the subject. This analysis could be augmented by AI tools capable of large-scale data processing and pattern recognition. Alternatively, the decision on the number and nature of perspectives could itself be a subject of debate, especially in a platform like SocraSynth, where different viewpoints can be represented and argued. This approach allows for a dynamic understanding of the subject, evolving with the discourse.

==> RelatedWork.tex <==
\section{Notes on Related Work}
\label{sec:related}

The advent of LLMs \cite{wolf2019transfertransfo,chatgpt} has been a watershed moment in the field of Natural Language Processing (NLP), demonstrating the enormous potential of large pre-trained language models (LLMs) coupled with prompting techniques. A recent survey by Google \cite{SocraticModels-Google2022} differentiates between basic and complex templates, the latter of which employ advanced strategies such as ensemble methods \cite{Schick2020ExploitingCF} for generating paraphrased prompts \cite{Haviv2021BERTeseLT}. For instance, works such as chain-of-thought  \cite{wei2022chain, ChainExtended2023}, tree-of-thought \cite{},  cumulative reasoning~\cite{}, and their incremental enhancements (e.g., \cite{PromptSurvey2023,jung2022maieutic,allaway2023penguins,sclar2023minding}) are complex templates that can support 
high-order logic reasoning with a limited set of truths.  
Higher-order logic is notably expressive and can represent many mathematical theories and concepts directly. However, this expressiveness comes at a computational cost when the involved truths may
be vast and even unbounded.
In the realm of generative and analytical tasks that require 
multidisciplinary domain knowledge and novel
knowledge discovery, SocraSynth is a pioneering work.


\begin{comment}
The existential quantifier in first-order logic is denoted by the symbol $\exists$, and is used to denote that there exists at least one element in the domain of discourse for which the proposition holds true. It doesn't convey a sense of quantity beyond the existence of at least one such element, so it does not specify whether ``some,'' ``a lot of,'' ``majority,'' or ``minority'' of elements satisfy the proposition.

For example, the statement $\exists x P(x)$ is read as ``There exists an $x$ such that $P(x)$ is true.'' It doesn’t provide any information about how many such $x$ exist that satisfy $P(x)$; it merely asserts that at least one such $x$ exists.

If you want to express concepts like ``some,'' ``most,'' or ``a lot of,'' you would typically need to use more expressive forms of logic or additional axioms and definitions that can capture these more nuanced quantitative concepts. For instance, to express ``most,'' you might define a predicate that is true when the majority of elements in a set satisfy a certain property and then use that predicate in conjunction with quantifiers to express your statement.

Higher-order logic is notably expressive and can represent many mathematical theories and concepts directly. However, this expressiveness comes at a computational cost. While first-order logic has a complete and sound proof system (thanks to the Gödel completeness theorem), higher-order logic does not enjoy such a property, and its decision problem is undecidable. Despite these complexities, higher-order logic finds applications in formal verification, theorem proving, and areas of artificial intelligence where expressiveness is crucial.
\end{comment}
